Basic Thresholding Classification

In this thesis, we propose a light-weight sparsity-based algorithm, basic thresholding classifier (BTC), for classification applications (such as face identification, hyper-spectral image classification, etc.) which is capable of identifying test samples extremely rapidly and performing high classification accuracy. Originally BTC is a linear classifier which works based on the assumption that the samples of the classes of a given dataset are linearly separable. However, in practice those samples may not be linearly separable. In this context, we also propose another algorithm namely kernel basic thresholding classifier (KBTC) which is a non-linear kernel version of the BTC algorithm. KBTC can achieve promising results especially when the given samples are linearly non-separable. For both proposals, we introduce sufficient identification conditions (SICs) under which BTC and KBTC can identify any test sample in the range space of a given dictionary. By using SICs, we develop parameter estimation procedures which do not require any cross validation. Both BTC and KBTC algorithms provide efficient classifier fusion schemes in which individual classifier outputs are combined to produce better classification results. For instance, for the application of face identification, this is done by combining the residuals having different random projectors. For spatial applications such as hyper-spectral image classification, the fusion is carried out by incorporating the spatial information, in which the output residual maps are filtered using a smoothing filter. Numerical results on publicly available face and hyper-spectral datasets show that our proposal outperforms well-known support vector machines (SVM)-based techniques, multinomial logistic regression (MLR)-based methods, and sparsity-based approaches like $l_1$-minimization and simultaneous orthogonal matching pursuit (SOMP).

==> codes/btc.tex <==
%\begin{lstlisting}
function [btcResult, errMatrix] = btc(labels, A, Y, M, alpha)
 % N represents the number of traning samples
 [~, N] = size(A);
 % L denotes the number of testing samples
 [~, L] = size(Y);
 % C shows the number of classes
 C = max(labels);
 % initialize the sparse codes for each test sample
 X = zeros(N, L);
 % calculate gram matrix, this can be performed outside the func
 mappedTrains = A' * A;
 % linear correlation vector is calculated for each test sample
 mappedAy = A' * Y;
 % correlation vectors are sorted in descending order
 [~, sortedLabels] = sort(abs(mappedAy), 'descend');
 % regularization matrix
 I = alpha * eye(M);
 % sparse code vector is calculated for each sample
 for k = 1:L
     % index set corresponding to the largest M correlations
     support = sortedLabels(1:M, k);
     % estimate sperse codes
     X(support, k) = (mappedTrains(support,support) + I) \ ...
     mappedAy(support,k);
 end
 % initialize error (residual) matrix
 errMatrix = zeros(C, L);
 % calculate class-wise regression error vector for each sample
 for classIndex = 1:C
     ind = (labels == classIndex);
     Yp = A(:,ind)*X(ind, :);
     errMatrix(classIndex,:) = sqrt(sum((Y-Yp).^2, 1));
 end
 % make decision for each sample based on minimum residual
 [~, btcResult] = min(errMatrix, [], 1);
 end
%\end{lstlisting}
